Tight Sampling in Unbounded Networks

The default approach to deal with the enormous size and limited accessibility of many Web and social media networks is to sample one or more subnetworks from a conceptually unbounded unknown network. Clearly, the extracted subnetworks will crucially depend on the sampling scheme. Motivated by studies of homophily and opinion formation, we propose a variant of snowball sampling designed to prioritize inclusion of entire cohesive communities rather than any kind of representativeness, breadth, or depth of coverage. The method is illustrated on a concrete example, and experiments on synthetic networks suggest that it behaves as desired.

==> files/fig_tex_files/1k_nodes_10in8_seeds_1_ratio.tex <==
\begin{figure*}[!ht] 
\centering 
\subfloat[\centering ][Evolution of network boundary with time]
{{\includegraphics[width=0.45\textwidth]{files/final_plots_rnr_v1/synthetic/1k_nodes_10in8_seeds_1_ratio/sbm_6.6.1_3_boundary.pdf}}}
% \subfloat[\centering ][Evolution of network boundary/outsider count with time]
% {{\includegraphics[width=0.33\textwidth]{files/final_plots_rnr_v1/synthetic/1k_nodes_10in8_seeds_1_ratio/sbm_6.6.1_3_boundary_by_outs.pdf}}}
\subfloat[\centering ][Community size evolution]
{{\includegraphics[width=0.45\textwidth]{files/final_plots_rnr_v1/synthetic/1k_nodes_10in8_seeds_1_ratio/sbm_6.6.1_3_comm_evol.pdf}}}
% \subfloat[\centering ][]


% \qquad 
% \subfloat[$\phi$ across all schemes] 
% {{\includegraphics[width=0.23\textwidth]{files/final_plots/conductance_dir_all_7.pdf}}}
% \subfloat[$Q$ across all schemes]
% {{\includegraphics[width=0.23\textwidth]{files/final_plots/modularity_all_7.pdf}}}
\caption{Sampling using MAS for a network of 8 blocks with 1000 nodes and 10 seed nodes each. The ratio of intra cluster to inter cluster edges ($r$) and average degree within the block are set as 1 and 10 respectively. Here, we are able to identify inflection points in (a) around timesteps 1000, 2000, 3000 etc. and observe that for the corresponding points in (b), there is a sharp increase in size of one community - indicating its sampling}
 \label{fig:sbm_1k_20in3_1_boundary_by_outs}
\end{figure*}
